A Computational Approach to Packet Classification

Multi-field packet classification is a crucial component in modern software-defined data center networks. To achieve high throughput and low latency, state-of-the-art algorithms strive to fit the rule lookup data structures into on-die caches; however, they do not scale well with the number of rules. We present a novel approach, NuevoMatch, which improves the memory scaling of existing methods. A new data structure, Range Query Recursive Model Index (RQ-RMI), is the key component that enables NuevoMatch to replace most of the accesses to main memory with model inference computations. We describe an efficient training algorithm that guarantees the correctness of the RQ-RMI-based classification. The use of RQ-RMI allows the rules to be compressed into model weights that fit into the hardware cache. Further, it takes advantage of the growing support for fast neural network processing in modern CPUs, such as wide vector instructions, achieving a rate of tens of nanoseconds per lookup. Our evaluation using 500K multi-field rules from the standard ClassBench benchmark shows a geometric mean compression factor of 4.9x, 8x, and 82x, and average performance improvement of 2.4x, 2.6x, and 1.6x in throughput compared to CutSplit, NeuroCuts, and TupleMerge, all state-of-the-art algorithms.

==> charts/iset_number_analysis-100k.tex <==

% ========================================================
% 100K classifiers
% ========================================================
\begin{axis}[
at={(0in,0in)},
ylabel={Time (ns)},
xlabel={Number of \isets in Classifier},
xmajorgrids, ymajorgrids, ymin=0, ymax=1000,
title={100k Classifiers}
]

% Remainder per iSet for 100k:
\addplot[draw=remainder,fill=remainder,opacity=0.6,area legend, postaction={pattern=dots,pattern color=remainder_pattern}] table{
0 403.126
1 212.724
2 118.251
3 120.749
4 104.106
5 115.119
6 112.425
} \closedcycle; \addlegendentry{Remainder};

% Search per iSet for 100k:
\addplot[fill=search, draw=search,opacity=0.6,area legend, postaction={pattern=north east lines,pattern color=search_pattern}] table{
0 403.126
1 269.332
2 205.05
3 235.5
4 246.384
5 288.953
6 312.046
% This is for completing the graph fill without overlapping
6 112.425
5 115.119
4 104.106
3 120.749
2 118.251
1 212.724
0 403.126
}; \closedcycle \addlegendentry{Binary Search};

% Validation per iSet for 100k:
\addplot[draw=validation,fill=validation,opacity=0.6,area legend,postaction={pattern=vertical lines,pattern color=validation_pattern}] table{
0 403.126
1 301.972
2 261.753
3 312.472
4 351.277
5 413.511
6 457.458
% This is for completing the graph fill without overlapping
6 312.046
5 288.953
4 246.384
3 235.5
2 205.05
1 269.332
0 403.126
} \closedcycle; \addlegendentry{Validation};

% Inference per iSet for 100k:
\addplot[fill=inference, draw=inference,opacity=0.6,area legend,postaction={pattern=crosshatch dots,pattern color=inference_pattern}] table{
0 403.126
1 344.843
2 344.039
3 419.342
4 485.434
5 569.239
6 642.001
% This is for completing the graph fill without overlapping
6 457.458
5 413.511
4 351.277
3 312.472
2 261.753
1 301.972
0 403.126
}; \closedcycle \addlegendentry{Inference};


% Do not remove - coverage legend
\addlegendimage{mark=x, color=coverage, mark size={\markWidth pt}}
\addlegendentry{Coverage}
\end{axis}

\begin{axis}[
at={(0in,0in)},
axis y line*=right,
ylabel={Coverage (\%)}, ymin=0, ymax=100,
]

% This chart goes to the second axis system
% Coverage per iSet for 100k:
\addplot[mark=x, mark options={}, mark size={\markWidth}, draw=coverage] table{
    0 0
    1 78.3478
    2 96.027
    3 97.5486
    4 98.4327
    5 98.8391
    6 99.0433
};

\end{axis}


==> deprecated_text.tex <==
\begin{comment}
\begin{figure}[t]
	\centering
	\include{rmi_evaluation}
	\caption{The RMI \cite{Kraska2018} computation process with multiple stages and submodels denoted as $m_{ij}$. The output of each stage is used for picking the submodel in the following stage. All submodels are fed with the same input. The first stage contains a single submodel. The output of the last stage serves as the computed value.}
	\label{fig:rmi_evaluation_process}
\end{figure}
\end{comment}



\begin{definition} [\MSNN submodel]

    Denote the output of a 3-layer fully-connected neural network as:
    \begin{equation} \nonumber
    N_{i,j}(x)= A\big( x \cdot \bm{w_1} + \bm{b_1}  \big) \times \bm{w_2} + b_2
    \end{equation}

	\noindent
	where $x$ is a scalar input, $\bm{w_1}, \bm{b_1}$ are the weight and bias row-vectors for layer $1$ (hidden layer), and $\bm{w_2}, b_2$ are the weight column-vector and bias scalar for layer $2$. Note that $N_{i,j}(x)$ is a scalar. The ReLU function $A$ applies a function $a$ on each element of an input vector:
	\begin{equation} \nonumber
	a(x)=
	\begin{cases} 
	x & x\geq0 \\
	0 & x<0.
	\end{cases} 
	\end{equation}
	
    \noindent
	The output of a submodel $m_{i,j}$, denoted $M_{i,j}(x)$,  is defined as follows:
	\begin{equation} \nonumber
	M_{i,j}(x)= H\big( N_{i,j}(x)\big)
	\end{equation}
	
	\noindent
	where $H(x)$ is a function which guarantees that the output domain is trimmed to $[0,1)$. 
	
	\begin{comment}
	Namely, for some $0<\delta \ll 1$, $M_{i,j}(x) \in [0, 1-\delta]$. Specifically:
	\begin{equation} \nonumber
	H(x)=
	\begin{cases} 
	0 & x<0 \\
	x & x \in [0,1-\delta) \\
	1-\delta & x \geq 1-\delta
	\end{cases} 
	\end{equation}
	\end{comment}
\end{definition}






% Alon: I leave it out, too much technical details.
\begin{comment}
\section{Validation Scheme} \label{appendix:validation}
The validation phase of \ouralgorithm{} enables it to scale well to any number of fields, as well as to support CMRs (see Appendix \ref{appendix:cmr}). Moreover, its design allows it to harness commodity vectorization engines available in modern CPUs for acceleration. Recall that different \isets perform separate validation phases (see figure \ref{fig:lookup_procedure}). As CMRs are a generalization of matching-rules, we denote the set of CMRs an \iset $i$ holds as $C_i$.

\begin{definition}[The Validation Phase's Height]
    Let $C_i$ be the set of CMRs of \iset $i$. We address the the validation phase of \iset $i$, and term its height as:
    \begin{equation*}
    h_i=\max{\Big\{\max{\{|E_j|\;\big\rvert\;E_j \in C\}}\;\Big\rvert\;C \in C_i\Big\}}
    \end{equation*}

\end{definition}

\begin{definition}[An Incoming Packet Matrix]
    Let $P$ be an incoming packet. Define the incoming packet matrix of $P$ of order $h_i \times F$ as
    
    \begin{equation*}
    \hat{P} = 
    \begin{pmatrix}
    p_0 & p_1 & \cdots & p_{F-1} \\
    p_0 & p_1 & \cdots & p_{F-1} \\
    \vdots & \vdots  & \ddots & \vdots \\
    p_0 & p_1 & \cdots & p_{F-1} \\
    \end{pmatrix}
    \end{equation*}
\end{definition}

\begin{definition}[CMR Matrices]
    Let $C=\big\{  E_0,\;E_1,\;E_2,\;...,\;E_{F-1}\big\} \in C_i$ be a CMR such that $E_f$ is a set of ranges $\big\{r_{f,j}\big\}_{j=0}^{|E_f|-1}$ that satisfy $C$ in field $f=\{0,1,2,...,F-1\}$. For completeness, we extend $\{r_{f,j}\}$ for all $f$ such that $\big\{r_{f,j}\big\}_{j=|E_f|-1}^{h_i}=\bot$. Denote $r_{f,j}=[a_{f,j},b_{f,j}]$. The lower-bound $\hat{C_l}$ and upper-bound $\hat{C_h}$ matrices of $C$, both of order $h_i \times F$, are defined as follows:
      
    \begin{equation*}
    \hat{C_l} = 
    \begin{pmatrix}
    a_{0,0} & a_{1,0} & \cdots & a_{F-1,0} \\
    a_{0,1} & a_{1,1} & \cdots & a_{F-1,1} \\
    \vdots & \vdots  & \ddots & \vdots \\
    a_{0,h_i} & a_{1,h_i} & \cdots & a_{F-1,h_i} \\
    \end{pmatrix}
    \end{equation*}

    \begin{equation*}
    \hat{C_h} =
    \begin{pmatrix}
    b_{0,0} & b_{1,0} & \cdots & b_{F-1,0} \\
    b_{0,1} & b_{1,1} & \cdots & b_{F-1,1} \\
    \vdots & \vdots  & \ddots & \vdots \\
    b_{0,h_i} & b_{1,h_i} & \cdots & b_{F-1,h_i} \\
    \end{pmatrix}
    \end{equation*}
    
\end{definition}

The validation phase checks whether an input packet $P$ satisfies (Definition \ref{rdefinition:cmr_match}) the secondary search's resulting candidate $C$ using a simple calculation over the matrices $\hat{P}, \hat{C_l}, \hat{C_h}$. More details are available in the source code of \ouralgorithm{}.
\end{comment}
